On the combinatorics of the refined 1-leg DT/PT correspondence

We provide a new proof of a result of Bessenrodt on the relation among the generating series of reversed plane partitions and skew plane partitions, motivated by the geometric DT/PT wallcrossing formula for local curves recently proved by the third author. This also recovers a result of Sagan. We moreover establish various new closed formulas for the weighted enumeration of reversed and skew plane partitions, proving a result dual to a theorem by Gansner, we find a new identity on the generating series counting internal and external hooks of a given Young diagram, and we combine the latter with Bessenrodt's theorem. Finally, we interpret our results as identities in the Fock space via the bosonic/fermionic formalism.

==> macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%% PROOFOF

\makeatletter
\newenvironment{proofof}[1]{\par
  \pushQED{\qed}%
  \normalfont \topsep6\p@\@plus6\p@\relax
  \trivlist
  \item[\hskip3\labelsep
        \itshape
    Proof of #1\@addpunct{.}]\ignorespaces
}{%
  \popQED\endtrivlist\@endpefalse
}
\makeatother


% Arrows
\DeclareSymbolFont{cmarrows}{OMS}{cmsy}{m}{n}
\SetSymbolFont{cmarrows}{bold}{OMS}{cmsy}{b}{n}
\DeclareMathSymbol{\cmminus}{\mathbin}{cmarrows}{"00}
\DeclareRobustCommand\relbar{\mathrel{\smash\cmminus}}
\DeclareMathSymbol{\leftrightarrow}{\mathrel}{cmarrows}{"24}
\DeclareMathSymbol{\leftarrow}{\mathrel}{cmarrows}{"20}
   \let\gets=\leftarrow
\DeclareMathSymbol{\rightarrow}{\mathrel}{cmarrows}{"21}
   \let\to=\rightarrow
\DeclareMathSymbol{\mapstochar}{\mathrel}{cmarrows}{"37}
   \def\mapsto{\mapstochar\rightarrow}

% Alphabets
\DeclareSymbolFont{usualmathcal}{OMS}{cmsy}{m}{n}
\DeclareSymbolFontAlphabet{\mathcal}{usualmathcal}
\DeclareMathAlphabet\BCal{OMS}{cmsy}{b}{n}

% Lists
\makeatletter
\newcommand{\mylabel}[2]{#2\def\@currentlabel{#2}\label{#1}}
\makeatother

% := per definizioni
\newcommand*{\defeq}{\mathrel{\vcenter{\baselineskip0.5ex \lineskiplimit0pt
                     \hbox{\scriptsize.}\hbox{\scriptsize.}}}=}
% colors
\definecolor{cornellred}{rgb}{0.7, 0.11, 0.11}
\definecolor{britishracinggreen}{rgb}{0.0, 0.26, 0.15}
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}

\usepackage{amsmath,float,soul}

\newcommand{\scat}{\scalebox{0.25}{\yng(1)}}
\newcommand{\QQuot}[2]{\Quot\left(\OO_{\BA^2}^{\oplus #1}, #2 \right)}
%\newcommand{\PP}[1]{\mathsf{P}_{#1}}
\newcommand{\ZZ}{\mathsf{Z}}
\newcommand{\QQ}{\mathsf{Q}}
\newcommand{\PP}{\mathsf{P}}
\newcommand{\pr}{\mathsf{pr}}
\newcommand{\Gr}{\mathrm{Gr}}
\newcommand{\BGr}{{\mathbb{G}\mathrm{r}}}
\newcommand{\dd}{\mathrm{d}}
\newcommand{\ob}{\mathrm{ob}}
\newcommand{\sm}{\mathrm{sm}}
\newcommand{\sing}{\mathrm{Sing}}
\newcommand{\sat}{\mathrm{sat}}
\newcommand{\mult}{\mathrm{mult}}
\newcommand{\Span}{\mathrm{Span}}
\newcommand{\codim}{\mathrm{codim}}
\newcommand{\simto}{\,\widetilde{\to}\,}
\newcommand{\into}{\hookrightarrow}
\newcommand{\onto}{\twoheadrightarrow}
\newcommand{\HH}{\mathrm{H}}
\newcommand{\Def}{\mathsf{Def}}
\newcommand{\OO}{\mathscr O}
\newcommand{\OF}{\mathscr F}
\newcommand{\OA}{\mathscr A}
\newcommand{\OC}{\mathscr C}
\newcommand{\OI}{\mathscr I}
\newcommand{\OG}{\mathscr G}
\newcommand{\OZ}{\mathscr Z}
\newcommand{\OW}{\mathscr W}
\newcommand{\OH}{\mathscr H}
\newcommand{\OM}{\mathscr M}
\newcommand{\OU}{\mathscr U}
\newcommand{\Ohom}{{\mathscr H}om}
\newcommand{\bfk}{\mathbf{k}}
\newcommand{\bfq}{\mathbf{q}}
\newcommand{\bfd}{\mathbf{d}}
\newcommand{\bfn}{\mathbf{n}}
\newcommand{\derived}{\mathbf{D}}
\newcommand{\BRPP}{\mathsf{RPP}}
\newcommand{\RF}{\mathsf{RF}}
\newcommand{\boldit}[1]{\boldsymbol{#1}}
\newcommand{\hilb}[2]{(\mathbb{P}^{#1})^{ [#2] } }
\newcommand{\CCoh}{\mathscr{C}\kern-0.25em {o}\kern-0.2em{h}}
\newcommand{\HHilb}{\mathcal{HILB}}




% bold + italics
\DeclareMathOperator{\bnu}{{\boldit{\nu}}} 
\DeclareMathOperator{\bn}{{\boldit{n}}}
\DeclareMathOperator{\Bm}{{\boldit{m}}}
\DeclareMathOperator{\bt}{{\boldit{t}}}
\DeclareMathOperator{\bh}{{\boldit{h}}}
\DeclareMathOperator{\be}{{\boldit{e}}}
\DeclareMathOperator{\ba}{{\boldit{a}}}
\DeclareMathOperator{\by}{{\boldit{y}}}
\DeclareMathOperator{\bk}{{\boldit{k}}}
\DeclareMathOperator{\bv}{{\boldit{v}}}
\DeclareMathOperator{\sep}{sep}
\DeclareMathOperator{\rpp}{rpp}
\DeclareMathOperator{\spp}{spp}
\DeclareMathOperator{\nes}{nes}
\DeclareMathOperator{\cones}{cones}
\DeclareMathOperator{\Syg}{Syg} 

\DeclareMathOperator{\vd}{vdim}
\DeclareMathOperator{\rk}{rk}
\DeclareMathOperator{\vir}{\mathrm{vir}}
\DeclareMathOperator{\sta}{\mathsf{st}}
\DeclareMathOperator{\free}{\mathsf{free}}
\DeclareMathOperator{\At}{\mathrm{At}}
\DeclareMathOperator{\Ind}{\mathrm{Ind}}
\DeclareMathOperator{\ord}{\mathrm{ord}}
\DeclareMathOperator{\Fact}{\mathrm{Fact}}
\DeclareMathOperator{\Subsoc}{\mathrm{Subsoc}}
\DeclareMathOperator{\Soc}{\mathrm{Soc}}
\DeclareMathOperator{\RPP}{\textsf{RPP}}
\DeclareMathOperator{\YF}{\textsf{YF}}
\DeclareMathOperator{\Hilb}{Hilb}
\DeclareMathOperator{\Exp}{Exp}
\DeclareMathOperator{\Philb}{P\mbox{-}Hilb}
\DeclareMathOperator{\Sym}{Sym}
\DeclareMathOperator{\chara}{char}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\Div}{Div}
\DeclareMathOperator{\GL}{GL}
\DeclareMathOperator{\In}{In}
\DeclareMathOperator{\colen}{colen}
\DeclareMathOperator{\Sat}{Sat}
\DeclareMathOperator{\Coh}{Coh}
\DeclareMathOperator{\Rep}{Rep}
\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\End}{End}
\DeclareMathOperator{\Ext}{Ext}
\DeclareMathOperator{\ncQuot}{ncQuot}
\DeclareMathOperator{\Quot}{Quot}
\DeclareMathOperator{\Mat}{Mat}
\DeclareMathOperator{\Orb}{Orb}
\DeclareMathOperator{\MHS}{MHS}
\DeclareMathOperator{\HS}{HS}
\DeclareMathOperator{\NW}{NW}
\DeclareMathOperator{\SW}{SW}
\DeclareMathOperator{\NE}{NE}
\DeclareMathOperator{\Aut}{Aut}
\DeclareMathOperator{\Spec}{Spec}
\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\Bl}{Bl}
\DeclareMathOperator{\Art}{Art}
\DeclareMathOperator{\Sets}{Sets}
\DeclareMathOperator{\SET}{SET}
\DeclareMathOperator{\red}{red}
\DeclareMathOperator{\length}{length}
\DeclareMathOperator{\opp}{op}
\DeclareMathOperator{\pt}{pt}
\DeclareMathOperator{\Sch}{Sch}
\DeclareMathOperator{\Supp}{Supp}
\DeclareMathOperator{\Bs}{Bs}
\DeclareMathOperator{\dP}{dP}

% alphabets
%\newcommand{\bh}{\mathbf{h}}
\newcommand{\TT}{\mathbf{T}}
\newcommand{\BA}{{\mathbb{A}}}
\newcommand{\BB}{{\mathbb{B}}}
\newcommand{\BC}{{\mathbb{C}}}
\newcommand{\BD}{{\mathbb{D}}}
\newcommand{\BE}{{\mathbb{E}}}
\newcommand{\BF}{{\mathbb{F}}}
\newcommand{\BG}{{\mathbb{G}}}
\newcommand{\BH}{{\mathbb{H}}}
\newcommand{\BI}{{\mathbb{I}}}
\newcommand{\BJ}{{\mathbb{J}}}
\newcommand{\BK}{{\mathbb{K}}}
\newcommand{\BL}{{\mathbb{L}}}
\newcommand{\BM}{{\mathbb{M}}}
\newcommand{\BN}{{\mathbb{N}}}
\newcommand{\BO}{{\mathbb{O}}}
\newcommand{\BP}{{\mathbb{P}}}
\newcommand{\BQ}{{\mathbb{Q}}}
\newcommand{\BR}{{\mathbb{R}}}
\newcommand{\BS}{{\mathbb{S}}}
\newcommand{\BT}{{\mathbb{T}}}
\newcommand{\BU}{{\mathbb{U}}}
\newcommand{\BV}{{\mathbb{V}}}
\newcommand{\BW}{{\mathbb{W}}}
\newcommand{\BX}{{\mathbb{X}}}
\newcommand{\BY}{{\mathbb{Y}}}
\newcommand{\BZ}{{\mathbb{Z}}}

\newcommand{\CA}{{\mathcal A}}
\newcommand{\CB}{{\mathcal B}}
\newcommand{\CC}{{\mathcal C}}
\newcommand{\CD}{{\mathcal D}}
\newcommand{\CE}{{\mathcal E}}
\newcommand{\CF}{{\mathcal F}}
\newcommand{\CG}{{\mathcal G}}
\newcommand{\CH}{{\mathcal H}}
\newcommand{\CI}{{\mathcal I}}
\newcommand{\CJ}{{\mathcal J}}
\newcommand{\CK}{{\mathcal K}}
\newcommand{\CL}{{\mathcal L}}
\newcommand{\CM}{{\mathcal M}}
\newcommand{\CN}{{\mathcal N}}
\newcommand{\CO}{{\mathcal O}}
\newcommand{\CP}{{\mathcal P}}
\newcommand{\CQ}{{\mathcal Q}}
\newcommand{\CR}{{\mathcal R}}
\newcommand{\CS}{{\mathcal S}}
\newcommand{\CT}{{\mathcal T}}
\newcommand{\CU}{{\mathcal U}}
\newcommand{\CV}{{\mathcal V}}
\newcommand{\CW}{{\mathcal W}}
\newcommand{\CX}{{\mathcal X}}
\newcommand{\CY}{{\mathcal Y}}
\newcommand{\CZ}{{\mathcal Z}}

\newcommand{\FA}{{\mathfrak{A}}}
\newcommand{\FB}{{\mathfrak{B}}}
\newcommand{\FC}{{\mathfrak{C}}}
\newcommand{\FD}{{\mathfrak{D}}}
\newcommand{\FE}{{\mathfrak{E}}}
\newcommand{\FF}{{\mathfrak{F}}}
\newcommand{\FG}{{\mathfrak{G}}}
\newcommand{\FH}{{\mathfrak{H}}}
\newcommand{\FI}{{\mathfrak{I}}}
\newcommand{\FJ}{{\mathfrak{J}}}
\newcommand{\FK}{{\mathfrak{K}}}
\newcommand{\FL}{{\mathfrak{L}}}
\newcommand{\FM}{{\mathfrak{M}}}
\newcommand{\FN}{{\mathfrak{N}}}
\newcommand{\FO}{{\mathfrak{O}}}
\newcommand{\FP}{{\mathfrak{P}}}
\newcommand{\FQ}{{\mathfrak{Q}}}
\newcommand{\FR}{{\mathfrak{R}}}
\newcommand{\FS}{{\mathfrak{S}}}
\newcommand{\FT}{{\mathfrak{T}}}
\newcommand{\FU}{{\mathfrak{U}}}
\newcommand{\FV}{{\mathfrak{V}}}
\newcommand{\FW}{{\mathfrak{W}}}
\newcommand{\FX}{{\mathfrak{X}}}
\newcommand{\FY}{{\mathfrak{Y}}}
\newcommand{\FZ}{{\mathfrak{Z}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\nested}[1]{(\BA^2)^{[#1]}}

%%%%%%%%%%%%%%%%%%%%%%%%%
%\usepackage[all]{xy}
\usepackage{tikz}
\usepackage{tikz-cd}
\usepackage{adjustbox}
\usepackage{rotating}
\usepackage{comment}
\newcommand*{\isoarrow}[1]{\arrow[#1,"\rotatebox{90}{\(\sim\)}"
]}
\usetikzlibrary{matrix,shapes,intersections,arrows,patterns,decorations.pathmorphing,decorations.markings}
%\tikzset{commutative diagrams/arrow style=math font}
\tikzset{commutative diagrams/.cd,
mysymbol/.style={start anchor=center,end anchor=center,draw=none}}
\newcommand\MySymb[2][\square]{%
  \arrow[mysymbol]{#2}[description]{#1}}
\tikzset{
shift up/.style={
to path={([yshift=#1]\tikztostart.east) -- ([yshift=#1]\tikztotarget.west) \tikztonodes}
}
}

\newcommand{\completion}[1]{\widetilde{#1}}

\newcommand{\cerchio}[2]{\begin{tikzpicture}
    \draw (0,0) circle (#2);
    \node at (0,-0.125) {$#1$};
\end{tikzpicture}}


%Sergej
\usepackage[enableskew]{youngtab} % youngtab want label with one entry, so I define some extra commands

\usepackage{ytableau} %better for the labelling
  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\theoremstyle{definition}

\newtheorem*{lemma*}{Lemma}
\newtheorem*{theorem*}{Theorem}
\newtheorem*{example*}{Example}
\newtheorem*{fact*}{Fact}
\newtheorem*{notation*}{Notation}
\newtheorem*{definition*}{Definition}
\newtheorem*{prop*}{Proposition}
\newtheorem*{remark*}{Remark}
\newtheorem*{corollary*}{Corollary}
\newtheorem*{solution}{Solution}
\newtheorem*{conventions*}{Conventions}

\newtheorem{definition}{Definition}[section]
\newtheorem{assumption}{Assumption}[section]
\newtheorem{problem}[definition]{Problem}
\newtheorem{example}[definition]{Example}
\newtheorem{fact}[definition]{Fact}
\newtheorem{conventions}[definition]{Conventions}
\newtheorem{convention}[definition]{Convention}
\newtheorem{question}[definition]{Question}
\newtheorem{notation}[definition]{Notation}
\newtheorem{notation-construction}[definition]{Notation-Construction}
\newtheorem{construction}[definition]{Construction}
\newtheorem{remark}[definition]{Remark}
\newtheorem{claim}[definition]{Claim}

\newtheorem{observation}[definition]{Observation}

\newtheoremstyle{thm} % <name> % (ambienti con dimostrazione)
        {3mm}% <Space above>
        {3mm}% <Space below>
        {\slshape}% <Body font> % 
        {0mm}% <Indent amount>
        {\bfseries}% <Theorem head font>
        {.}% <Punctuation after theorem head>
        {1mm}% <Space after theorem head>
        {}% <Theorem head spec (can be left empty, meaning 'normal')> 
\theoremstyle{thm}
\newtheorem{theorem}[definition]{Theorem}
\newtheorem{corollary}[definition]{Corollary}
\newtheorem{lemma}[definition]{Lemma}
\newtheorem{prop}[definition]{Proposition}
\newtheorem{conjecture}[definition]{Conjecture}

\newtheorem{thm}{Theorem}
\renewcommand*{\thethm}{\Alph{thm}}
\newcommand{\ledot}{\begin{tikzcd}
<\hspace{-0.15cm}\raisebox{0.05cm}{$\scriptscriptstyle\bullet$}
\end{tikzcd}}
\newcommand{\gedot}{\begin{tikzcd}
\raisebox{0.05cm}{$\scriptscriptstyle\bullet$}
\end{tikzcd}\hspace{-0.3cm}>}

\newcommand{\linkesempi}{da mettere}


%Ser
\newtheorem*{Acknowledgments*}{Acknowledgments}


%%%%%%%%%% TARTAGLIA %%%%%%%%%%%%%

\newcommand{\motive}[1]{ \left[ #1 \right]
}

\newcommand{\tartaglia}[1]{
\begin{tikzpicture}
\foreach \i in {0,...,{#1}}
    \foreach \j in {0,...,\i}
            \pgfmathtruncatemacro{\ciao}{factorial(\i)/(factorial(\j)*factorial(\i-\j))}
	       \node at ( \j*0.8-\i/2*0.8,-\i*0.8) {\ciao};
\end{tikzpicture}
}

\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}


\renewcommand{\geq}{\geqslant}
\renewcommand{\ge}{\geqslant}
\renewcommand{\leq}{\leqslant}
\renewcommand{\le}{\leqslant}

\newcommand{\FFQ}{\ensuremath{\mathsf{FQ}}}
\newcommand{\FFZ}{\ensuremath{\mathsf{FZ}}}


%Sergej
\newcommand{\RR}{{\mathbf{R}}}

